Core Decomposition in Multilayer Networks: Theory, Algorithms, and Applications

Multilayer networks are a powerful paradigm to model complex systems, where multiple relations occur between the same entities. Despite the keen interest in a variety of tasks, algorithms, and analyses in this type of network, the problem of extracting dense subgraphs has remained largely unexplored so far. In this work we study the problem of core decomposition of a multilayer network. The multilayer context is much challenging as no total order exists among multilayer cores; rather, they form a lattice whose size is exponential in the number of layers. In this setting we devise three algorithms which differ in the way they visit the core lattice and in their pruning techniques. We then move a step forward and study the problem of extracting the inner-most (also known as maximal) cores, i.e., the cores that are not dominated by any other core in terms of their core index in all the layers. Inner-most cores are typically orders of magnitude less than all the cores. Motivated by this, we devise an algorithm that effectively exploits the maximality property and extracts inner-most cores directly, without first computing a complete decomposition. Finally, we showcase the multilayer core-decomposition tool in a variety of scenarios and problems. We start by considering the problem of densest-subgraph extraction in multilayer networks. We introduce a definition of multilayer densest subgraph that trades-off between high density and number of layers in which the high density holds, and exploit multilayer core decomposition to approximate this problem with quality guarantees. As further applications, we show how to utilize multilayer core decomposition to speed-up the extraction of frequent cross-graph quasi-cliques and to generalize the community-search problem to the multilayer setting.

==> brain.tex <==
%!TEX root = tkdd_revision.tex

\subsection{Core decomposition of neuroimages to study the effects of LSD on the human brain}
Recently there has been a surge of interest in modeling the brain as a graph and complex topological and functional properties as graph problems \cite{sporns2005human}.
We apply the techniques developed in this paper to the analysis of a dataset of neuroimages that have been used to study the effect of \emph{lysergic acid diethylamide} (LSD) on the human brain \cite{carhart2016neural}. The dataset is based on three different and complementary neuroimaging techniques: \emph{arterial spin labeling} (ASL), \emph{blood oxygen level-dependent} (BOLD) measures, and \emph{magnetoencephalography} (MEG), implemented during resting state conditions. For each individual of the 15 partecipating in the study, the three neuroimaging techniques are used in two different states: under placebo and under LSD effect.
Each neuroimage, after adequate processing \cite{carhart2016neural}, produces a graph with 165 vertices.

We created 6 multilayer networks, one for each neuroimaging technique and for each of the two states. All the multilayer networks have 15 layers corresponding to the 15 different individuals.  We applied core decomposition to the 6 multilayer networks.

\begin{figure}[h!]
\centering
\begin{tabular}{rccc}  
 & \hspace{-2mm} \textsf{ASL} & \hspace{-2mm}\textsf{BOLD} & \hspace{-2mm}\textsf{MEG}\\
 \begin{turn}{90} $\; \; \; \; \; \; \; \; \; \;$ \textsf{LSD} \end{turn} &
\hspace{-2mm} \includegraphics[width=.16\textwidth]{figures/lsd_15_res1.pdf} &
\hspace{-4mm} \includegraphics[width=.16\textwidth]{figures/lsd_15_res2.pdf} &
\hspace{-4mm} \includegraphics[width=.16\textwidth]{figures/lsd_15_res3.pdf}  \\
 \begin{turn}{90} $\; \; \; \; \; \; \;$ \textsf{Placebo}\end{turn} & 
\hspace{-2mm} \includegraphics[width=.16\textwidth]{figures/pcb_15_res1.pdf} & 
\hspace{-4mm} \includegraphics[width=.16\textwidth]{figures/pcb_15_res2.pdf} & 
\hspace{-4mm} \includegraphics[width=.16\textwidth]{figures/pcb_15_res3.pdf}\\
\end{tabular}
\caption{Distribution of number of cores per level for the 6 multilayer networks in the neuroimages database. \label{fig:brain}}
\end{figure}





\subsection{Co-authorship networks}
\note[Francesco]{Not sure we will have this one.
}


